Considerations on supersymmetric Dark Matter beyond the MSSM

The standard model (SM) of particle physics is for the last three decades a very successful description of the properties and interactions of all known elementary particles. Currently, it is again probed with the first collisions at the Large Hadron Collider (LHC). It is widely expected that new physics will be detected at the LHC and the SM has to be extended. The most exhaustive analyzed extension of the SM is supersymmetry (SUSY). SUSY can not only solve intrinsic problems of the SM like the hierarchy problem, but it also postulates new particles which might explain the nature of dark matter in the universe. The majority of all studies about dark matter in the framework of SUSY has focused on the minimal supersymmetric standard model (MSSM). The aim of this work is to consider scenarios beyond that scope. We consider two models which explain not only dark matter but also neutrino masses: the gravitino as dark matter in gauge mediated SUSY breaking (GMSB) with bilinear broken R-parity as well as different seesaw scenarios with the neutralino as dark matter candidate. Furthermore, we also study the next-to-minimal supersymmetric standard model (NMSSM) which solves the (\mu)-problem of the MSSM and discuss the properties of the neutralino as dark matter candidate.

==> Feynmangraphen/feynmf.1 <==
.\" Automatically generated by Pod::Man v1.37, Pod::Parser v1.14
.\"
.\" Standard preamble:
.\" ========================================================================
.de Sh \" Subsection heading
.br
.if t .Sp
.ne 5
.PP
\fB\\$1\fR
.PP
..
.de Sp \" Vertical space (when we can't use .PP)
.if t .sp .5v
.if n .sp
..
.de Vb \" Begin verbatim text
.ft CW
.nf
.ne \\$1
..
.de Ve \" End verbatim text
.ft R
.fi
..
.\" Set up some character translations and predefined strings.  \*(-- will
.\" give an unbreakable dash, \*(PI will give pi, \*(L" will give a left
.\" double quote, and \*(R" will give a right double quote.  | will give a
.\" real vertical bar.  \*(C+ will give a nicer C++.  Capital omega is used to
.\" do unbreakable dashes and therefore won't be available.  \*(C` and \*(C'
.\" expand to `' in nroff, nothing in troff, for use with C<>.
.tr \(*W-|\(bv\*(Tr
.ds C+ C\v'-.1v'\h'-1p'\s-2+\h'-1p'+\s0\v'.1v'\h'-1p'
.ie n \{\
.    ds -- \(*W-
.    ds PI pi
.    if (\n(.H=4u)&(1m=24u) .ds -- \(*W\h'-12u'\(*W\h'-12u'-\" diablo 10 pitch
.    if (\n(.H=4u)&(1m=20u) .ds -- \(*W\h'-12u'\(*W\h'-8u'-\"  diablo 12 pitch
.    ds L" ""
.    ds R" ""
.    ds C` ""
.    ds C' ""
'br\}
.el\{\
.    ds -- \|\(em\|
.    ds PI \(*p
.    ds L" ``
.    ds R" ''
'br\}
.\"
.\" If the F register is turned on, we'll generate index entries on stderr for
.\" titles (.TH), headers (.SH), subsections (.Sh), items (.Ip), and index
.\" entries marked with X<> in POD.  Of course, you'll have to process the
.\" output yourself in some meaningful fashion.
.if \nF \{\
.    de IX
.    tm Index:\\$1\t\\n%\t"\\$2"
..
.    nr % 0
.    rr F
.\}
.\"
.\" For nroff, turn off justification.  Always turn off hyphenation; it makes
.\" way too many mistakes in technical documents.
.hy 0
.if n .na
.\"
.\" Accent mark definitions (@(#)ms.acc 1.5 88/02/08 SMI; from UCB 4.2).
.\" Fear.  Run.  Save yourself.  No user-serviceable parts.
.    \" fudge factors for nroff and troff
.if n \{\
.    ds #H 0
.    ds #V .8m
.    ds #F .3m
.    ds #[ \f1
.    ds #] \fP
.\}
.if t \{\
.    ds #H ((1u-(\\\\n(.fu%2u))*.13m)
.    ds #V .6m
.    ds #F 0
.    ds #[ \&
.    ds #] \&
.\}
.    \" simple accents for nroff and troff
.if n \{\
.    ds ' \&
.    ds ` \&
.    ds ^ \&
.    ds , \&
.    ds ~ ~
.    ds /
.\}
.if t \{\
.    ds ' \\k:\h'-(\\n(.wu*8/10-\*(#H)'\'\h"|\\n:u"
.    ds ` \\k:\h'-(\\n(.wu*8/10-\*(#H)'\`\h'|\\n:u'
.    ds ^ \\k:\h'-(\\n(.wu*10/11-\*(#H)'^\h'|\\n:u'
.    ds , \\k:\h'-(\\n(.wu*8/10)',\h'|\\n:u'
.    ds ~ \\k:\h'-(\\n(.wu-\*(#H-.1m)'~\h'|\\n:u'
.    ds / \\k:\h'-(\\n(.wu*8/10-\*(#H)'\z\(sl\h'|\\n:u'
.\}
.    \" troff and (daisy-wheel) nroff accents
.ds : \\k:\h'-(\\n(.wu*8/10-\*(#H+.1m+\*(#F)'\v'-\*(#V'\z.\h'.2m+\*(#F'.\h'|\\n:u'\v'\*(#V'
.ds 8 \h'\*(#H'\(*b\h'-\*(#H'
.ds o \\k:\h'-(\\n(.wu+\w'\(de'u-\*(#H)/2u'\v'-.3n'\*(#[\z\(de\v'.3n'\h'|\\n:u'\*(#]
.ds d- \h'\*(#H'\(pd\h'-\w'~'u'\v'-.25m'\f2\(hy\fP\v'.25m'\h'-\*(#H'
.ds D- D\\k:\h'-\w'D'u'\v'-.11m'\z\(hy\v'.11m'\h'|\\n:u'
.ds th \*(#[\v'.3m'\s+1I\s-1\v'-.3m'\h'-(\w'I'u*2/3)'\s-1o\s+1\*(#]
.ds Th \*(#[\s+2I\s-2\h'-\w'I'u*3/5'\v'-.3m'o\v'.3m'\*(#]
.ds ae a\h'-(\w'a'u*4/10)'e
.ds Ae A\h'-(\w'A'u*4/10)'E
.    \" corrections for vroff
.if v .ds ~ \\k:\h'-(\\n(.wu*9/10-\*(#H)'\s-2\u~\d\s+2\h'|\\n:u'
.if v .ds ^ \\k:\h'-(\\n(.wu*10/11-\*(#H)'\v'-.4m'^\v'.4m'\h'|\\n:u'
.    \" for low resolution devices (crt and lpr)
.if \n(.H>23 .if \n(.V>19 \
\{\
.    ds : e
.    ds 8 ss
.    ds o a
.    ds d- d\h'-1'\(ga
.    ds D- D\h'-1'\(hy
.    ds th \o'bp'
.    ds Th \o'LP'
.    ds ae ae
.    ds Ae AE
.\}
.rm #[ #] #H #V #F C
.\" ========================================================================
.\"
.IX Title "FEYNMF 1"
.TH FEYNMF 1 "1996-12-02" "FeynMF Version 1.08" "Contributed LaTeX Utilities"
.SH "NAME"
\&\fBfeynmf\fR \- Process \fBLaTeX\fR files using \fBFeynMF\fR
.SH "SYNOPSIS"
.IX Header "SYNOPSIS"
\&\fBfeynmf\fR [\fB\-hvqncfT\fR] [\fB\-t\fR \fItfm\fR [\fB\-t\fR \fItfm\fR ...]] [\fB\-m\fR \fImode\fR]
       \fIfile\fR [\fIfile\fR ...]
.PP
\&\fBfeynmf\fR [\fB\-\-help\fR] [\fB\-\-version\fR] [\fB\-\-quiet\fR] [\fB\-\-noexec\fR] [\fB\-\-clean\fR]
       [\fB\-\-force\fR] [\fB\-\-notfm\fR] [\fB\-\-tfm\fR \fItfm\fR [\fB\-\-tfm\fR \fItfm\fR ...]]
       [\fB\-\-mode\fR \fImode\fR] \fIfile\fR [\fIfile\fR ...]
.SH "DESCRIPTION"
.IX Header "DESCRIPTION"
The most complicated part of using the \fBFeynMF\fR style appears to be the
proper invocation of \fBMetafont\fR.  The \fBfeynmf\fR script provides a
convenient front end and will automagically invoke \fBMetafont\fR with the
proper mode and magnifincation.  It will also avoid cluttering system font
directories and offers an option to clean them.
.SH "OPTIONS"
.IX Header "OPTIONS"
.IP "\fB\-h\fR, \fB\-\-help\fR" 4
.IX Item "-h, --help"
Print a short help text.
.IP "\fB\-v\fR, \fB\-\-version\fR" 4
.IX Item "-v, --version"
Print the version of \fBfeynmf\fR.
.IP "\fB\-q\fR, \fB\-\-quiet\fR" 4
.IX Item "-q, --quiet"
Don't echo the commands being executed.
.IP "\fB\-n\fR, \fB\-\-noexec\fR" 4
.IX Item "-n, --noexec"
Don't execute \fBLaTeX\fR or \fBMetafont\fR.
.IP "\fB\-c\fR, \fB\-\-clean\fR" 4
.IX Item "-c, --clean"
Offer to delete font files that have accidentally been placed in a
system directory by the \fBMakeTeXTFM\fR and \fBMakeTeXPK\fR scripts (these
scripts are run by \fBtex\fR (and \fBlatex\fR) in the background).  This
option has only been tested with recent versions of \s-1UNIX\s0 TeX.
.IP "\fB\-f\fR, \fB\-\-force\fR" 4
.IX Item "-f, --force"
Don't ask any questions.
.IP "\fB\-T\fR, \fB\-\-notfm\fR" 4
.IX Item "-T, --notfm"
Don't try to prepare fake \f(CW\*(C`.tfm\*(C'\fR files for the first run.
.IP "\fB\-t\fR, \fB\-\-tfm\fR \fItfm\fR" 4
.IX Item "-t, --tfm tfm"
Don't try guess the names of the \f(CW\*(C`.tfm\*(C'\fR files to fake for
the first run and use the given name(s) instead.  This option
can be useful if our incomplete parsing of the LaTeX input
files fails.
.IP "\-\fBm\fR \fImode\fR, \fB\-\-mode\fR \fImode\fR" 4
.IX Item "-m mode, --mode mode"
Select the \s-1METAFONT\s0 mode \fImode\fR.  The default is guessed or
\&\f(CW\*(C`localfont\*(C'\fR if the guess fails.
.IP "\fIfile\fR" 4
.IX Item "file"
Main \fBLaTeX\fR input files.
.IP "\fIfile\fR ..." 4
.IX Item "file ..."
Other LaTeX input files that are included by the main file.
.SH "AUTHOR"
.IX Header "AUTHOR"
Thorsten Ohl <Thorsten.Ohl@Physik.TH\-Darmstadt.de>
.SH "BUGS"
.IX Header "BUGS"
The preparation of \f(CW\*(C`.tfm\*(C'\fR files is not foolproof yet, because we can
parse \fBTeX\fR files only superficially.
.PP
This script has only been tested for recent \fBteTeX\fR distributions
of \s-1UNIX\s0 \fBTeX\fR, though it will probably work with other versions of
\&\s-1UNIX\s0 \fBTeX\fR.  The author will be grateful for portability suggestions,
even concerning \fBBorg\fR operating systems, for the benefit of those users
that are forced to live with \s-1DOS\s0 or Windows.


==> TeX/empty.tex <==
\newpage


==> TeX/erklaerung.tex <==
\chapter*{Erkl\"arung}
\addcontentsline{toc}{chapter}{Erkl\"arung}

Diese Doktorarbeit wurde am Lehrstuhl f\"ur Theoretische Physik II,
Theoretische Elementarteilchenphysik, der
Julius-Maximilians-Universit\"at W\"urzburg angefertigt.

Ich erkl\"are hiermit, dass ich diese Dissertation selbst\"andig verfasst und keine anderen als die angegebenen Quellen und Hilfsmittel benutzt habe.\\
Ich erkl\"are au{\ss}erdem, dass diese Dissertation weder in gleicher noch in anderer Form bereits in einem anderen Pr\"ufungsverfahren vorgelegen hat.\\
Ich habe fr\"uher au{\ss}er den mit dem Zulassungsgesuch urkundlich vorgelegten Graden keine weiteren akademischen Grade erworben oder zu erwerben versucht. 

\vspace{3cm}

\begin{flushleft}
 \begin{picture}(100,5)
 \line(1,0){170} 
 \end{picture}
\vspace{0.3cm}\\
 Florian Staub \\
 W\"urzburg, den XX. September 2010
\end{flushleft}



==> TeX/relic.tex <==
\chapter{Relic Density}
\label{chapter:relic}
Since the derivation of the Lee-Weinberg formula from the Boltzmann equation is often skipped in literature, we want to give the most important steps here. This derivation was presented by Prof. Stefano Scopel at the ISAPP summer school 2008 in Madrid. \\
The starting point is the Boltzmann equation
\begin{equation}
L[f] = C[f]
\end{equation}
Here, \(f\) is a function of \(x^\mu, p^\mu\) and the time \(t\). The phase space density only depends on \(E\) and therefore we get
\begin{equation}
 f(x^\mu, p^\mu, t) = f(E,t) \thickspace ,
\end{equation}
and the WIMP number density is \(n(t) = \frac{g}{(2 \pi)^3} \int d^3 \vec{p} f(E,t)\) \thickspace .
We can write the Liouville operator as
\begin{equation}
L = \frac{d}{d \tau} = p^\mu \frac{d}{d x\mu} - \Gamma^\mu_{\sigma \rho} p^\sigma p^\rho \frac{d}{d p^\mu}
\end{equation}
by using the definition of the proper time \(d \tau = \sqrt{-g^{\mu\nu} d x_\mu x_\nu}\), the action for a free particle \(A = - \dot{\tau}\) and the background force term from the geodesic equation
\begin{equation}
\frac{d p^\mu}{d \tau} = - \Gamma^\mu_{\sigma \rho} p^\sigma p^\rho \thickspace .
\end{equation}
We have a dependence on gravitational background through affine connection
\begin{equation}
\Gamma^\sigma_{\lambda \mu} = \frac{1}{2} \left(\frac{\partial g_{\mu\nu}}{\partial x^\lambda}+\frac{\partial g_{\lambda\nu}}{\partial x^\mu} - \frac{\partial g_{\mu\lambda}}{\partial x^\nu} \right)  \thickspace .
\end{equation}
Restricting to Robertson Walker metric
\begin{equation}
d s^2 = d t^2 - a^2(t) \left(\frac{d r^2}{1 - k r^2} + r^2 d \Theta + r^2 \sin^2 \Theta d\phi^2 \right) \thickspace .
\end{equation}
the only non zero-terms are
\begin{eqnarray}
 \Gamma^i_{jk} &=& \frac{1}{2} h^{il} \left(\frac{\partial g_{lj}}{\partial x^k} + \frac{\partial g_{lk}}{\partial x^j} - \frac{\partial g_{jk}}{\partial x^l} \right) \\
\Gamma^0_{ij} &=& \frac{\dot{a}}{a} h_{ij} = H h_{ij} \\
\Gamma^i_{0 j} &=& \frac{\dot{a}}{a} \delta^i_j
\end{eqnarray}
with \(h_{ij}\) as the \(3 \times 3\) unit matrix. By defining the entropy density \(s = \frac{\rho + }{T}=g_s \frac{2 \pi^2}{45} T^3\) and using for the yield \(Y = \frac{n}{s}\)
\begin{equation}
\frac{d Y}{d t} = \frac{d}{dt} \left(\frac{Y}{s}\right) = \frac{1}{s} \left( \frac{dn}{dt} + 3 H n \right)
\end{equation}
we get from a integration over the phase space
\begin{equation}
\frac{g}{(2 \pi)^3} \int \frac{d^3 \vec{p}}{E} L[f] = \frac{d n}{dt} + 3 H n = s \frac{d Y}{dt} \thickspace .
\end{equation}
The next step is to consider the collision operator. Therefore we define \(d \Pi_i = \frac{g_i}{2 \pi^3} \frac{d^3 p_i}{2 E_i}\), where \(g_i\) are the internal degrees of freedom. A phase space integration for the annihilation of two WIMPs \(a,b\) into to light SM particles \(1,2\) reads as
\begin{equation}
\label{collision}
\frac{g}{(2 \pi)^3} \int C[f] \frac{d^3 \vec{p}}{E} = - \int  d\Pi_1 d\Pi_2 d\Pi_a d\Pi_b (2 \pi)^4 \delta^4(p_1+p_2-p_a-p_b)\left(|M_{12\rightarrow ab}|^2 f_1 f_2 - |M_{ab-> 12}|^2 f_a f_b \right) \thickspace .
\end{equation}
We can simplify this by assuming that the SM particles are in thermal equilibrium
\begin{equation}
f_{a,b} = f^{eq}_{a,b} = e^{\frac{E_{a,b}}{T}}
\end{equation}
and by demanding detailed balance
\begin{equation}
f_a^{eq} f^{eq}_b = e^{\frac{E_a+E_b}{T}} = e^{\frac{E_1+E_2}{T}} = f^{eq}_1 f^{eq}_2 \thickspace .
\end{equation}
The thermal averaged annihilation cross section is
\begin{equation}
\bra \sigma v \ket = \frac{1}{n_{eq}^2} \int d\Pi_1 d\Pi_2 d\Pi_a d\Pi_b (2 \pi)^4 \delta^4 (p_1+p_2-p_a - p_b) |M|^2 f_1^{eq} f_2^{eq} 
\end{equation}
and the result of eq.~(\ref{collision}) is
\begin{equation}
 \frac{g}{(2 \pi)^3} \int C[f] \frac{d^3 \vec{p}}{E} = - \bra \sigma v \ket \left(n^2 - n_{eq}^2\right) \thickspace .
\end{equation}

Putting the pieces together, we derive out of the Boltzmann's equation the Lee-Weinberg formula for the number density
\begin{equation}
\dot{n} + 3 H n = - \bra \sigma |v| \ket  \left(n^2 - n_{eq}^2 \right),
\end{equation}
or for the yield
\begin{equation}
\dot{Y} = -s \bra \sigma v \ket \left(Y^2 - Y^2_{eq}\right).
\end{equation}
This can also written as 
\begin{equation}
\frac{d Y}{d x} = -\frac{x s}{H(T=m)} \bra \sigma v \ket \left(Y^2 - Y^2_{eq}\right)
\end{equation}
by defining the freeze out parameter \(x = \frac{m}{T}\) and is known as Riccati equation. 

For \(x > x_f\) we get a separable equation
\begin{equation}
 \frac{d Y}{d x} = -\frac{x s}{H(T=m)} \bra \sigma v \ket Y^2 
\end{equation}
with the analytic solution
\begin{equation}
\frac{1}{Y_0} - \frac{1}{Y_f} \simeq \frac{1}{Y_0} = \sqrt{\frac{\pi}{45 G}} m \int_{x_0}^{x_f} \sqrt{g_*} \bra \sigma v \ket d\left(\frac{1}{x}\right)
\end{equation}
which can be simplified for non relativistic particles by using an expansion in \(x\)
\begin{equation}
\bra \sigma  v \ket \simeq a + \frac{b}{x} 
\end{equation}
to
\begin{equation}
\frac{1}{Y_0} \simeq \sqrt{\frac{\pi}{45 G}} \sqrt{g_*(T_f)} \frac{m}{x_f} \left(a+\frac{b}{2 x_f}  \right).
\end{equation}
% Finally, the thermal cosmological density of a WIMP is given by 
% \begin{equation}
% \Omega h^2 \sim \frac{1}{\bra \sigma v \ket_{int}}
% \end{equation}
% with \(\bra \sigma v\ket_{int} = \int_{x_f}^{x_0} \bra \sigma v \ket d x\). By inserting the today's entropy \(S_0 = 2970 \mbox{cm}^{-3}\), the critical density \(\rho_c = 1.054 10^{-5} \frac{\GeV}{\mbox{cm}^3}\), the freeze out parameter \(x_f \sim 20\), the number of degrees of freedom \(\sqrt{g_*} \sim 10\) and the Hubble parameter \(h=\frac{H_0}{100} km s^{-1} Mpc^{-1}\) we get for the WIMP density
% \begin{equation}
% \Omega_{\mbox{WIMP}} h^2 \simeq \frac{0.1 \mbox{pbarn}}{\bra \sigma v \ket}. 
% \end{equation}
The WIMP relic density is finally
\begin{equation}
\Omega_\chi h^2 = \frac{1.07 \cdot 10^9\, \mbox{GeV}^{-1}}{M_P} \frac{x_f}{\sqrt{g_*}} \frac{1}{a+3 b/x_f} \thickspace .
\end{equation}






